Density Based Outlier Scoring on Kepler Data

In the present era of large scale surveys, big data presents new challenges to the discovery process for anomalous data. Such data can be indicative of systematic errors, extreme (or rare) forms of known phenomena, or most interestingly, truly novel phenomena which exhibit as-of-yet unobserved behaviors. In this work we present an outlier scoring methodology to identify and characterize the most promising unusual sources to facilitate discoveries of such anomalous data. We have developed a data mining method based on k-Nearest Neighbor distance in feature space to efficiently identify the most anomalous lightcurves. We test variations of this method including using principal components of the feature space, removing select features, the effect of the choice of k, and scoring to subset samples. We evaluate the peformance of our scoring on known object classes and find that our scoring consistently scores rare (<1000) object classes higher than common classes. We have applied scoring to all long cadence lightcurves of quarters 1 to 17 of Kepler's prime mission and present outlier scores for all 2.8 million lightcurves for the roughly 200k objects.

==> sections/a_extra.tex <==
% Unused math
% It is convenient to organize this set as the vertical set of all feature vectors, $\mathbfss{F}_v$, which are the positions of each object in feature space, and the horizontal set of all feature sets, $\mathbfss{F}_h$.
% \begin{equation}\label{eq:featureMatrix2}
%     \mathbfss{F}_v = 
%     \begin{bmatrix}
%         \mathbfit{F}_1 \\
%         \vdots \\
%         \mathbfit{F}_N
%     \end{bmatrix},\\
%     \mathbfss{F}_h = 
%     \begin{bmatrix}
%         \mathbfit{f}_1 & \dots & \mathbfit{f}_M
%     \end{bmatrix}.
% \end{equation}\\

\subsection{PCA Reduction}
\label{results:PCA-red}
% might strike this section for the paper, it's useful for comparing
% the previous binary outlier determinations, but is reliant on now
% features which have been corrected and now deprecated methods.
% TODO: choose whether or not to keep this section.
Our initial exploration following the previous work was to explore the utility of dimensionality reduction both to improve computational performance and to reduce the exaggerated importance of correlated features. 

For an initial comparison with updated methods and feature definitions, and to evaluate the effects of random sampling, we re-performed the analysis on the un-reduced data to create a baseline of comparison. The new analysis produced significantly fewer outlier identifications for each quarter than the previous work. For reasons that are not immediately evident, performing the analysis with the same methodology produced a more conservative value for epsilon. Since the issue appears to be self-consistent at least, we proceed by providing a comparison of the baseline to the previous work, and compare reduced data to the baseline produced here as well as the previous work.

Essentially all outliers identified after reprocessing the data and after reductions were identified as such in the previous work, the precision of the new baseline and reductions is essentially 100\% when compared to the previous work. The recall, however, is between 50\% and 80\%. One goal of the previous work was to avoid any false negatives, i.e. missed outliers. The new results indicate a more selective set. 
Given the nature of our previous work to utilize more exclusive clustering parameters so that we would encompass all possible outliers, we favor the precision metric in evaluating the performance of these reductions against the previous work. We note the recall is very high when compared to the new baseline, but we cannot comment on the differences between reductions and baseline.

Compared to the baseline, i.e. treating the baseline as the ground truth, the reductions performed similarly. Both precision and recall were in the high 80s to 90s.

To explain 90\% of the variance required 17-18 dimensions. The time, t, for reduction and clustering varied between $5<t<7$ minutes.

To explain 95\% of the variance required 22-24 dimensions. The time, t, to reduce and cluster varied between $5.5<t<7.5$ minutes

To explain 99\% of the variance required 34-36 dimensions. The reduction and clustering required $7<t<9.5$ minutes.

We cannot directly evaluate the quality of outlier detection without prior knowledge of the underlying `truth', instead we characterize the differences in identifications between reductions.

% Other PCA section similar to above?
In our original work, we used a conservative cluster definition to produce a catalog of outliers with a focus on avoiding false negatives, rather than false positives (i.e. misidentifying outlying data as normal).
Our initial evaluation calculates the precision and recall of outlier identifications using the different reductions as compared to the previous proof-of-concept work, which is treated as ground truth. The conservative nature of our previous work is intended to capture all potential outliers, and as such we evaluate performance of changes in terms of the quality of outliers lost and percentage of outliers retained. 

PCA90 required between 14 and 18 components, PCA95 between 18 and 24, and PCA99 between 27 and 36 to explain their respective variances. Their times to reduce were 13.8$\pm$1.8s for PCA90, 20.8$\pm$2.8s for PCA95, and 35.6$\pm$4.8s for PCA99 on average.
The times to cluster were 373.7$\pm$68.0s, 444.1$\pm$77.5s, 546.6$\pm$88.0s.
\begin{table} 
	\centering
	\caption{A table describing the computational performance of the different reductions.}
	Times are averages across all quarters, error is the standard deviation.
	\label{tab:PCA_performance}

	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		Reduction & Dimensions & Time to Reduce & Time to Cluster\\
		& & s & s\\
		\hline
		Baseline & 60 & N/A & 780\\ %TODO: Get the times for baseline
		PCA90 & 16 & 13.8$\pm$1.8 & 373.8$\pm$68.0\\
		PCA95 & 21 & 20.8$\pm$2.8 & 444.1$\pm$77.5\\
		PCA99 & 32 & 35.6$\pm$4.8 & 546.6$\pm$88.0\\
		\hline
	\end{tabular}
\end{table}
%TODO: Produce average times for baseline
In addition to this evaluation as compared to previous work, we examine differences produced by PCA reductions on scoring in Section~\ref{scoring:parameters}.

\section{Overly detailed changes}
The most major corrections adjust the calculation of peak, and valley, statistics to center the peak, or valley, where they were previously offset from an index misassignment. 
We have also changed the assignment of dummy values in the case of divide-by-zero errors for the ratios of flatness and roundness measures of peaks to valleys. The asymmetry of maxima and minima for nonzero minima was discovered to greatly exceed the dummy values previously used in very rare We have changed the assignment of filler values in the case of divide-by-zero errors for the ratios of flatness and roundness of peaks to valleys. The asymmetry of maxima and minima for nonzero minima was discovered to greatly exceed the filler values previously used in rare cases (on the order of 1:$10^5$ lightcurves).
In this case of divide-by-zero errors, the lightcurve can have maxima and minima solely situated exactly at the edges of the lightcurve. 
Maxima and minima on the edges of lightcurves are not used in the calculation of peak (or valley) symmetry calculations since they do not have data on both sides of the extrema. If there are no other peaks or valleys in a lightcurve, the divide-by-zero error can occur when comparing the  average shapes of peaks to valleys. 
This issue is caught during feature calculation and issued a large dummy value with appropriate sign. The dummy values are chosen such that they would be much greater than ordinal data, but within orders of magnitude of the most extreme data that don't run into errors. 
We could have removed any objects which ran into this issue and flagged them automatically as outliers, but we are hesitant to remove any objects from the database, even in such extreme circumstances. Without presuming to know the population of the database, it was unknown whether this would be a common or uncommon issue. Instead, the dummy value was estimated to be reasonably extreme while still being within an order of magnitude of other potential data. 
% \begin{figure}\label{fig:edge-anomaly}
% 	\includegraphics[width=\columnwidth]{Plots/KIC11701418.png}
%     \caption{An anomalous lightcurve with a singular peak on the edge.}
% \end{figure}
% \begin{figure}\label{fig:longperiod}
% 	\includegraphics[width=\columnwidth]{Plots/KIC4671249.png}
%     \caption{A long period variable with an infinite roundness ratio, there are no minima so it is impossible to calculate the roundness of peaks to valleys.}
% \end{figure}
\section{Univariate Extreme Value Analysis}
In univariate extreme value analysis, the convention is to consider any point 1.5 times the interquartile range beyond the 25th or 75th percentile an outlier \citep{Aggarwal2013}. Applying this definition to the \krange{4}{14} k-average scores, we find that an outlier score of 0.00274 demarcates the boundary between normal and outlying data. This heuristic identifies 14,648 of the scores as outlying. In the same way, for PCA90 the score is 0.00365 with 13,497 outliers, PCA 95  0.00438 with 14,094, and PCA99 0.00599 with 15,206. Of these, 11,559 are outliers common to each reduction. By this heuristic measure, over 90\% of the data have consistently negligible scores. 

\begin{figure}
	\includegraphics[width=\columnwidth]{Plots/PCA_ranks.pdf}
    \caption{Examining the ranks of the 2k most outlying objects, more outlying being ranked higher and sorted from left to right, we see that ranks are mostly consistent with few major deviations when utilizing dimensionality reduction, despite significant variation in scores from the different reductions. As the data becomes less outlying, there is more variation in rank as a result of the tightly clustered nature of ordinal data.}
    \label{fig:PCA_rank}
\end{figure}

\subsection{Performance Improvements}
\label{results:performance}
In the interest of applying these methods to larger data sets, the methodology has been improved from previous iterations both in terms of speed and utility. 
The calculation of features is optimized to process features in under one quarter of the time per quarter, with even greater gains on individual lightcurves. For reference, the time to process all 156,126 of Quarter 1 lightcurves into features on 16 2.70GHz CPUs was 0:48:44.67 (hh:mm:ss), whereas previously the time to process a quarter *was longer than that.* %TODO: find these numbers and write this section.

\begin{figure*}
    \centering
    \includegraphics[width=2\columnwidth]{Plots/boyajians_lc.png}
    \caption{Light curve of Boyajian's star illustrating anomalous dips. \citep[Figure 1]{Boyajian2016}}
    \label{fig:boyajians_lc}
\end{figure*}

\begin{figure*}
	\includegraphics[width=2\columnwidth]{Plots/Boyajian_scores.png}
    \caption{Scores for Boyajian's star (KIC 8462852) across all Kepler quarters. The scores are k-average \krange{4}{14} scores, sampled 10\x 1k and scaled with reference to a sinusoid.}
    \label{fig:boyajian_scores}
\end{figure*}

\begin{itemize}
  \item 5944707 - EX, variable
  \item 7446357 - GO(various), Dwarf Nova
  \item 7199774 - EX and GO, Algol
  \item 9594451 - STC, none
  \item 7446357 - GO(various), dwarf nova
  \item 8451871 -  GO20031, none
  \item 5262664 - EX, None
  \item 100003607 - None, None
  \item 7199037 - EX and GO, Eruptive Variable
  \item 8415928 - GO(various), Dwarf nova
  \item 10057002 - GO40030, High proper motion star 
  \item 11199438 - EX, none
 \end{itemize}
